DAWN-ICL: Strategic Planning of Problem-solving Trajectories for Zero-Shot In-Context Learning

Zero-shot in-context learning (ZS-ICL) aims to conduct in-context learning (ICL) without using human-annotated demonstrations. Most ZS-ICL methods use large language models (LLMs) to generate (input, label) pairs as pseudo-demonstrations and leverage historical pseudo-demonstrations to help solve the current problem. They assume that problems are from the same task and traverse them in a random order. However, in real-world scenarios, problems usually come from diverse tasks, and only a few belong to the same task. The random traversing order may generate unreliable pseudo-demonstrations and lead to error accumulation. To address this problem, we reformulate ZS-ICL as a planning problem and propose a Demonstration-aware Monte Carlo Tree Search (MCTS) approach (DAWN-ICL), which leverages MCTS to strategically plan the problem-solving trajectories for ZS-ICL. In addition, to achieve effective and efficient Q value estimation, we propose a novel demonstration-aware Q-value function and use it to enhance the selection phase and accelerate the expansion and simulation phases in MCTS. Extensive experiments demonstrate the effectiveness and efficiency of DAWN-ICL on in-domain and cross-domain scenarios, and it even outperforms ICL using human-annotated labels. The code is available at https://github.com/RUCAIBox/MCTS4ZSICL.

==> sections/formulation.tex <==
\section{Problem Formulation}
\label{sec-formulation}

Zero-shot in-context learning~(ZS-ICL)~\cite{} enables task adaptation of LLMs at test time without using human-labeled examples as the demonstration.
Formally, given an LLM $M$ and a set of test examples $\mathcal{E} = \{(x_i, y_i)\}_{i=1}^n$, ZS-ICL first constructs pseudo-demonstration $d_i = F_M (x_i, \{d_j\}_{j=1}^{i-1})$ for the current input $x_i$ based on previous pseudo-demonstrations $\{d_j\}_{j=1}^{i-1}$, and then predicts the label $\hat{y}_i = G_M (x_i, d_i)$ with the newly constructed pseudo-demonstration $d_i$.

In existing work~\cite{}, the test examples are assumed to belong to the same task, and the example to solve at each step ($x_i$) is usually randomly selected.
However, in real-world scenarios, test examples come from diverse tasks and only a few examples belong to the same task, which makes it hard for task adaptation since task examples are limited.
To solve this, one feasible way is to leverage the examples from other tasks for solving the current task examples.
For this method, the key is to plan the order of solving the example set $\mathcal{E}$ since different examples may have significant differences and not be beneficial for the current one.

To this end, we can conceptualize the solving process of ZS-ICL as a Markov Decision Process~(MDP) by the tuple 


However, previous approaches often randomly select samples from the target task $T$, resulting in limited exploration of the problem space.
Therefore, to guide the LLM in actively selecting problems to solve, we frame the navigation of problem-solving paths as a strategy planning problem, which aims to determine the optimal sequence from a vast space of potential orders.
In this planning framework, we define the state $s \in \mathcal{S}$ as the set of problems that have been solved with pseudo labels predicted by ${F}$.
The action $a \in \mathcal{A}$ is a deterministic process that adds a new unsolved problem to the solved problem set and utilizes ICL with pseudo demonstrations to generate the answer.

After defining state and action, we can conceptualize the ZS-ICL process as a Markov Decision Process~(MDP) $⟨\mathcal{S},\mathcal{A},\mathcal{T},\mathcal{R},\gamma⟩$.
Here, the deterministic state transition $\mathcal{T}: \mathcal{S} \times \mathcal{A} \mapsto \mathcal{S}$ describes how we move from the current state $s_t$ to the next state $s_{t+1}$ by applying an action $a_t$, which involves adding a new problem to the current state and using ICL to make a prediction.
The reward function $\mathcal{R}$ measures the accuracy of the generated answers of $F$ for the current problem and the discount factor $\gamma$ is to balance exploration and exploitation.
% which we approximate using confidence by subtracting the probability of random guess from the probability of the generated label. 放到下一章说

